Devising a Set of Compact and Explainable Spoken Language Feature for Screening Alzheimer's Disease

Alzheimer's disease (AD) has become one of the most significant health challenges in an aging society. The use of spoken language-based AD detection methods has gained prevalence due to their scalability due to their scalability. Based on the Cookie Theft picture description task, we devised an explainable and effective feature set that leverages the visual capabilities of a large language model (LLM) and the Term Frequency-Inverse Document Frequency (TF-IDF) model. Our experimental results show that the newly proposed features consistently outperform traditional linguistic features across two different classifiers with high dimension efficiency. Our new features can be well explained and interpreted step by step which enhance the interpretability of automatic AD screening.

==> Section/6.Limitations.tex <==
\section{Limitaions}

==> Tables/prompts1.tex <==
\begin{longtable}{@{\extracolsep{\fill}}p{4cm}p{12cm}@{}}

\toprule
\textbf{Feature name} & \textbf{Prompt} \\
\midrule
\endfirsthead

\toprule
\textbf{Feature name} & \textbf{Prompt} \\
\midrule
\endhead

\bottomrule
\endfoot

\bottomrule
\endlastfoot

Feature Name 1 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Analyze the semantic repetition in the provided transcript of a 'Cookie Theft' picture description. Examine how the description revisits the same topics or concepts with different or similar phrasing, and provide a single numeric score that reflects the degree of semantic repetition. A higher score indicates more significant semantic repetition. 

High Repetition Score Example: "Can I start? There's a boy and the boy is reaching, the boy is reaching into the cookie jar. He's on the stool and reaching. His sister, she's next to him, waiting, just waiting. The water is overflowing, the water spills as the mother washes, she washes the dishes. The jar is on the counter, and the boy is on a stool." Output: 8.5. Explanation: This narrative repetitively emphasizes the boy’s focus on the cookies and the mother’s distraction, effectively illustrating how the same themes/topics are repeated. 

Low Repetition Score Example: "The boy stands on a stool reaching for a cookie jar while his sister watches quietly. Their mother is at the sink, washing dishes, unaware of the water spilling onto the floor from the overflowing sink." Output: 2. Explanation: This example receives a low score because it contains minimal repetition, indicating a more controlled and focused use of language, which is typical of cognitively healthy individuals. Remember your output should be strictly a single number as the last token without any explanations. \\
\hline
Feature Name 2 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Assess the structural complexity of the provided transcript describing the 'Cookie Theft' picture. Focus on the grammatical structure complexity of utterances and output a single numeric score where a higher score suggests higher structural complexity.
High Structural Complexity Score Example: "While the boy carefully stands on a stool reaching up to grab a cookie from the top shelf, his sister quietly watches every move, signaling him to be careful. At the same time, their mom, busy washing dishes at the sink, doesn't notice the water overflowing and spreading across the kitchen floor." Output: 7.5. Explanation: This example retains a complex narrative structure through the simultaneous description of multiple actions involving different subjects. It uses straightforward language but preserves the complexity by detailing the interactions and unawareness of different characters in a connected sequence of events.
Low Structural Complexity Score Example: "Boy on stool. He is stealing cookies.  Girl watches boy. Mother washes dishes." Output: 3. This example scores low due to its simplistic and fragmented sentence structure, lacking conjunctions and complex phrases. It shows minimal linguistic depth and reduced sentence complexity.
Remember your output should be strictly a single number as the last token without any explanations. \\
\hline
Feature Name 3 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Evaluate the referential specificity in the transcript of a 'Cookie Theft' picture description. Determine how specifically the descriptions refer to elements of the picture and output a single numeric score reflecting referential specificity, where a higher score suggests more specified reference to the picture.
High Specificity Score Example: "The boy, perched on a small wooden stool, reaches towards a glass cookie jar atop countertop. His sister, stands beside him, her index finger pressed to her lips. In the background, their mother, focuses on washing a pile of plates, unaware of the water spilling from sink." Output: 8. Explanation: Precise and detailed descriptions contribute to a clear and vivid depiction.
Low Specificity Score Example: "A kid is trying to get some cookies while another kid watches. She is doing the dishes." Output: 2.5. Explanation: Vague and generalized descriptions lead to an unclear and generic portrayal.
Remember your output should be strictly a single number as the last token without any explanations. \\
\hline
Feature Name 4 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Assess the coherence of the provided transcript describing the 'Cookie Theft' picture. Evaluate how logically and smoothly ideas are connected within the narrative. Provide a single numeric score reflecting the coherence of the language used, where a higher score indicates better coherence.
High Coherence Score Example: "In a lively kitchen scene, a young boy carefully balances on a stool as he reaches into a cookie jar located on the top shelf. Beside him, his sister silently signals caution with her gestures, closely observing his actions. Their mother, engaged in washing dishes, remains oblivious to the overflowing sink beside her, which is spilling water onto the clean kitchen floor." Output: 9.5. Explanation: This example receives a high score for coherence because the narrative flows logically and smoothly from one event to the next. The sequence of actions is clear, and the description effectively connects the actions of each family member, creating a cohesive and vivid scene.
Low Coherence Score Example: "The boy, something about reaching for a cookie or maybe he was just standing there. The sister, was she helping him? No, maybe she was playing or doing something else. There’s water, and it’s spilling, or maybe it was already there. The mother, I think she’s around, possibly cooking or cleaning, but it’s all a bit unclear what she’s focused on." Output: 3.5. Explanation: This narrative is scored low on coherence due to its disjointed and unclear progression. The description is vague, with uncertain and contradictory statements that disrupt the logical flow, making it difficult to follow or visualize the scene accurately.
Remember your output should be strictly a single number as the last token without any explanations. \\
\hline
Feature Name 5 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Examine the provided transcript for semantic impairments in the description of the 'Cookie Theft' picture. Analyze inaccuracies or impairments of language usage and provide a single numeric score representing the level of semantic impairment.
High Semantic Impairment Score Example: "The boy, standing by the oven, pulls plates from the refrigerator. His sister eats a spoon. Their mother is gardening the sink with water plants." Output: 9. Explanation: This example is rated highly for semantic impairments due to nonsensical phrases and incorrect word usage, such as 'gardening the sink' and 'eats a spoon', which indicate significant semantic errors and confusion.
Low Semantic Impairment Score Example: "The boy reaches into the cookie jar on the kitchen counter as his sister looks on, and their mother washes dishes." Output: 2.5.Explanation: This transcript is scored low for semantic impairments as it contains accurate and appropriate use of terms that correctly describe the actions and setting, showing clear semantic understanding.
Remember your output should be strictly a single number as the last token without any explanations. \\
\hline
Feature Name 6 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Assess the transcript describing the 'Cookie Theft' picture for evidence of short-term memory lapses. Analyze how the participant’s memory affects their ability to describe the scene consistently and output a single numeric score indicating the presence of memory lapses, where a higher score suggests more severe memory lapse.
High Memory Lapse Score Example: "The boy, uh, he's doing something by the sink... or no, he's getting cookies, and I think the water is running somewhere. There's a girl too, or maybe she was the mother?" Output: 8.5. Explanation: This example is scored high due to evident confusion and uncertainty about the events being described, reflecting possible memory lapses as the narrator struggles to recall and consistently describe the scene.
Low Memory Lapse Score Example: "The boy reaches into the cookie jar while standing on a stool, as his sister watches him and their mother washes dishes, unaware of the overflowing sink." Output: 2. Explanation: This example receives a low score because it shows a clear and consistent recollection of the events, with no indications of memory difficulty.
Remember your output should be strictly a single number as the last token without any explanations.\\
\hline
Feature Name 7 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Analyze the transcript describing the 'Cookie Theft' picture for linguistic deficits or atypical patterns that are suggestive of cognitive decline. Focus on identifying irregularities such as incorrect word use, incomplete sentences, or unusual phrasing. Output a single numeric score that quantifies the severity of these linguistic deficits, where a higher score suggests more severe deficits.
High Deficit Score Example: "Boy take cookie when no falling down. Girl look but no speaking. Water make floor wet while mother dish washing." Output: 8.5. Explanation: This example receives a high score due to the presence of grammatical errors and unusual phrasing, such as 'Boy take cookie when no falling down' and 'Water make floor wet'. These errors and the simplification of language structures suggest linguistic deficits typical of cognitive decline.
Low Deficit Score Example: "The young boy carefully reaches for cookies above him, while his sister quietly observes, and their mother busily washes the dishes, not noticing the overflowing sink." Output: 2. Explanation: This narrative is scored low because it is well-constructed, with correct grammar and appropriate use of language. There are no signs of linguistic deficits or atypical patterns, indicating a healthy linguistic ability.
Remember your output should be strictly a single number as the last token without any explanations. \\
\hline
Feature Name 8 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Assess the tangentiality of the provided transcript describing the 'Cookie Theft' picture. Provide a single numeric score reflecting the tangentiality of the transcript, where a higher score suggests the transcript contains more irrelevant information about the 'Cookie Theft' picture.
High Tangentiality Score Example: "Well, the boy is getting a cookie, but have you noticed how cookies are always so sweet? Speaking of sweet, I remember my grandmother used to make the best apple pies on sunny days just like today. Oh, and the sink is overflowing." Output: 9. Explanation: This example is rated high for tangentiality because the narrative quickly deviates from the main topic. The introduction of unrelated memories about sweetness and apple pies distracts from the primary scene, demonstrating a lack of focus and relevance, which are signs of cognitive issues.
Low Tangentiality Score Example: "The boy, standing on a stool, is reaching into a cookie jar. His sister watches him while their mother washes dishes, unaware of the overflowing sink." Output: 1.5. Explanation: This example receives a low tangentiality score because it maintains focus on the primary scene without straying into unrelated topics. Each sentence is relevant to the described situation, demonstrating clear and focused thought processes.
Remember your output should be strictly a single number as the last token without any explanations.\\
\hline
Feature Name 9 & Imagine you are an AI developed for medical diagnostics specializing in detecting signs of dementia. Assess the uncertainty of the provided transcript describing the 'Cookie Theft' picture. Provide a single numeric score reflecting the uncertainty of the transcript, where a higher score suggests the transcript is more uncertain about the 'Cookie Theft' picture.
High Uncertainty Score Example: "I think there might be a boy reaching for a cookie jar. It's hard to tell if he’s actually going to take a cookie or just looking inside. I'm not really sure what his intentions are. There’s also a woman—maybe his mother?—standing nearby, and it looks like she could be washing dishes, but I can’t say for certain because she might just be standing there. Is the water overflowing? It’s difficult to determine from this angle." Output: 7.5. Explanation: This narrative scores highly on the uncertainty scale due to numerous expressions of doubt and speculation. Phrases such as 'I think', 'it’s hard to tell', 'I’m not really sure', 'maybe', 'I can’t say for certain', and 'it’s difficult to determine' all contribute to a strong sense of uncertainty about the actions and the context of the scene.
Low Uncertainty  Score Example: "There is clearly a boy who is standing on a stool and reaching into a cookie jar placed on a high shelf. His sister is watching him quietly from the side, ensuring he doesn't fall. Their mother is at the sink, washing dishes, aware of the overflowing water, which she seems to be addressing by turning off the tap." Output: 3. Explanation: This example receives a low uncertainty score because the description is very direct and contains clear, confident statements about the scene. Phrases such as 'clearly', 'ensuring', 'completely aware' convey a high degree of certainty about the actions and the setting. There is no ambiguity or speculation present indicated by words such as  'maybe', indicating a strong sense of sureness about the details described.
Remember your output should be strictly a single number as the last token without any explanations. \\

\end{longtable}

\caption{Your Table Caption Here}
\label{tab:your_label}
